Searching for Effective Neural Network Architectures for Heart Murmur Detection from Phonocardiogram

Aim: The George B. Moody PhysioNet Challenge 2022 raised problems of heart murmur detection and related abnormal cardiac function identification from phonocardiograms (PCGs). This work describes the novel approaches developed by our team, Revenger, to solve these problems. Methods: PCGs were resampled to 1000 Hz, then filtered with a Butterworth band-pass filter of order 3, cutoff frequencies 25 - 400 Hz, and z-score normalized. We used the multi-task learning (MTL) method via hard parameter sharing to train one neural network (NN) model for all the Challenge tasks. We performed neural architecture searching among a set of network backbones, including multi-branch convolutional neural networks (CNNs), SE-ResNets, TResNets, simplified wav2vec2, etc. Based on a stratified splitting of the subjects, 20% of the public data was left out as a validation set for model selection. The AdamW optimizer was adopted, along with the OneCycle scheduler, to optimize the model weights. Results: Our murmur detection classifier received a weighted accuracy score of 0.736 (ranked 14th out of 40 teams) and a Challenge cost score of 12944 (ranked 19th out of 39 teams) on the hidden validation set. Conclusion: We provided a practical solution to the problems of detecting heart murmurs and providing clinical diagnosis suggestions from PCGs.

==> main.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Compiler: pdfLaTeX
% TeX Live version: 2022
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% unofficial phase abstract
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{contents/unofficial_abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% conference short paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{paper_short}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% conference poster
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{poster}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% long paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{paper_long}


==> tables/challenge_score_full.tex <==

\begin{table}[!htp]
\centering
% requires packages boldline, multirow
\setlength\tabcolsep{1pt}
\begin{tabular}{@{\extracolsep{4pt}}llllll@{}}
\hlineB{3.5}
 & & \multicolumn{2}{c}{Murmur} & \multicolumn{2}{c}{Outcome} \\ \cline{3-4} \cline{5-6}
 & & Score & Ranking & Score & Ranking \\
\hline
\multirow{3}{*}{Wt. Acc.} & Test & \textbf{0.736} & \textbf{14 / 40} & 0.761 & 10 / 39 \\
 & Validation & 0.678 & 20 / 40 & 0.671 & 16 / 39 \\
 & Training & 0.757 & 26 / 40 & 0.77 & 29 / 39 \\ \hline
\multirow{3}{*}{Cost} & Test & 19476 & 33 / 40 & \textbf{12944} & \textbf{19 / 39} \\
 & Validation & 13552 & 25 / 40 & 10647 & 21 / 39 \\
 & Training & 18109 & 34 / 40 & 12244 & 32 / 39 \\ \hline
\multirow{3}{*}{Accuracy} & Test & 0.843 & 2 / 40 & 0.52 & 30 / 39 \\
 & Validation & 0.805 & 8 / 40 & 0.436 & 33 / 39 \\
 & Training & 0.856 & 19 / 40 & 0.52 & 35 / 39 \\
F-measure & Test & 0.559 & 18 / 40 & 0.442 & 34 / 39 \\
 & Validation & 0.536 & 21 / 40 & 0.414 & 34 / 39 \\
 & Training & 0.568 & 28 / 40 & 0.453 & 35 / 39 \\ \hline
\multirow{3}{*}{AUROC} & Test & 0.776 & 20 / 40 & 0.594 & 19 / 39 \\
 & Validation & 0.698 & 30 / 40 & 0.603 & 17 / 39 \\
 & Training & 0.768 & 32 / 40 & 0.616 & 32 / 39 \\ \hline
\multirow{3}{*}{AUPRC} & Test & 0.611 & 17 / 40 & 0.604 & 18 / 39 \\
 & Validation & 0.582 & 23 / 40 & 0.601 & 17 / 39 \\
 & Training & 0.614 & 30 / 40 & 0.61 & 32 / 39 \\
\hlineB{3.5}
\end{tabular}
\caption{to write.}
\label{tab:challenge_scores_full}
\end{table}

